Designing Autonomous Markets for Stablecoin Monetary Policy

We develop a new type of automated market maker (AMM) that helps to maintain stability and long-term viability in a stablecoin. This primary market AMM (P-AMM) is an autonomous mechanism for pricing minting and redemption of stablecoins in all possible states and is designed to achieve several desirable properties. We first cover several case studies of current ad hoc stablecoin issuance and redemption mechanisms, several of which have contributed to recent stablecoin de-peggings, and formulate desirable properties of a P-AMM that support stability and usability. We then design a P-AMM redemption curve and show that it satisfies these properties, including bounded loss for both the protocol and stablecoin holders. We further show that this redemption curve is path independent and has properties of path deficiency in extended settings involving trading fees and a separate minting curve. This means that system health weakly improves relative to the path independent setting along any trading curve and that there is no incentive to strategically subdivide redemptions. Finally, we show how to implement the P-AMM efficiently on-chain.

==> content/6-time_dependency.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Behavior across Multiple Blocks}\label{sec:time-dependency}

We now consider a different extension of the redemption curve across multiple blocks.
Recall that our system so far has assumed that all trades occur within a single block so that the state $x_0$ at the beginning of the block is just a constant.
Across blocks, $x_0$ captures the \emph{outflow history}, i.e., the time-discounted amount of redemptions that have occurred so far. Thus, a large amount of redemptions within any given block will increase the value that $x_0$ takes in the next block. If no such redemptions happen, $x_0$ decays and takes on a smaller value in the next block.

[This section is currently work in progress. Results to be proven: (i) As $x_0$ decreases, $\rho$ increases all else equal. This means that traders who do not have urgency redeeming are always better off waiting until the outflow history has decayed over time. This is another useful price-stabilizing property of the mechanism. We have checked this numerically and it shouldn't be hard to prove formally. (ii) Characterize how quickly this happens, i.e., characterize sensitivity of $r_L$ to decay in $x_0$]


